An Analytical Framework for Control Synthesis of Cyber-Physical Systems with Safety Guarantee

Cyber-physical systems (CPS) are required to operate safely under fault and malicious attacks. The simplex architecture and the recently proposed cyber resilient architectures, e.g., Byzantine fault tolerant++ (BFT++), provide safety for CPS under faults and malicious cyber attacks, respectively. However, these existing architectures make use of different timing parameters and implementations to provide safety, and are seemingly unrelated. In this paper, we propose an analytical framework to represent the simplex, BFT++ and other practical cyber resilient architectures (CRAs). We construct a hybrid system that models CPS adopting any of these architectures. We derive sufficient conditions via our proposed framework under which a control policy is guaranteed to be safe. We present an algorithm to synthesize the control policy. We validate the proposed framework using a case study on lateral control of a Boeing 747, and demonstrate that our proposed approach ensures safety of the system.

==> PPC.tex <==
\section{Prescribed Performance Control Based Synthesis}

Define a finite time performance function $p(t)$ whose dynamics are given as
\begin{equation}
    \dot{p}=-\varepsilon p(t)^\kappa,
\end{equation}
where $\varepsilon>0$, $\kappa\in(0,1)$ are parameters. The solution $p(t)$ is given as
\begin{equation}
    p(t)=\begin{cases}
    (p(0)^{1-\kappa}-\varepsilon(1-\kappa)t)^{1/(1-\kappa)}+p_\infty,&~\forall t\in[0,T)\\
    p_\infty,&~\forall t\in[T,\infty)
    \end{cases}
\end{equation}
where $p_\infty\geq 0$, $T=\frac{p(0)^{1-\kappa}}{\varepsilon(1-\kappa)}$ is the finite convergent time.

Suppose the budget cost when the system reaches the normal state is $cB$ where $c\in(0,1]$. Define
\begin{subequations}\label{eq:remaining budget time domain}
\begin{align}
    e(t) &= cB - J(t,x)\\
    \xi(t) &= \frac{e(t)}{p(t)}\\
    \epsilon(t) & = S(\xi(t))=\ln\left(\frac{\xi(t)}{1-\xi(t)}\right)
\end{align}
\end{subequations}
Here $e(t)$ captures the remaining budget for the normal state during one cyber cycle, $\xi(t)$ is the normalized remaining budget during the normal state, $\epsilon(t)$ is the transformed remaining budget. We then have the following dynamics to describe the evolution of $e(t)$, $\xi(t)$, and $\epsilon(t)$:
\begin{subequations}
\begin{align}
    \dot{e} &= -\frac{\partial J}{\partial x}(x)(f(x)+g(x)u)\\
    \dot{\xi} &= \frac{\dot{e}p(t)-e(t)\dot{p}}{p(t)^2}=\frac{1}{p(t)}(\dot{e}-\xi(t)\dot{p})\\
    \dot{\epsilon} &= \frac{1-\xi(t)}{\xi(t)}\frac{1-\xi(t)+\xi(t)}{(1-\xi(t))^2}\dot{\xi}=\frac{\dot{e}-\xi(t)\dot{p}}{p(t)\xi(t)(1-\xi(t))}
\end{align}
\end{subequations}

Our goal is to guarantee that
\begin{equation}
    0<e(t)<p(t)
\end{equation}
holds during the normal state. Using the definitions in Eqn. \eqref{eq:remaining budget time domain}, the goal is converted to the problem to guaranteeing $\epsilon(t)$ to be bounded.

Denote the initial system state of the normal state as $x_0$.
\begin{lemma}\label{lemma:existence of maximal sol}
Assume that $\xi(0,x_0)\in\Xi=(0,1)$ and control input $u$ is determined by a continuous and bounded control law. There exists a maximal solution $\xi(t)$ such that $\xi(t)\in \Xi$ for all $t\in[0,\tau_{\max})$.
\end{lemma}
\begin{proof}
We prove the lemma using Lemma \ref{lemma:maximal sol}. Define $y=[x^\top,\xi]^\top$. Then the dynamics of $y$ are given as
\begin{equation*}
    \dot{y} = F(t,y)=\begin{bmatrix}f(x)+g(x)u\\
    \frac{1}{p(t)}(\dot{e}-\xi(t)\dot{p})
    \end{bmatrix}=\begin{bmatrix}F_1(t,y)\\
    F_2(t,y)
    \end{bmatrix}
\end{equation*}
By our assumption, we have that $\xi(0,x_0)\in\Xi=(0,1)$. Let $\Omega_x(t)=\{x:\xi(t,x)\in(0,1)\}$. Since $\Xi$ is a non-empty and open set, we have that the inverse image $\Omega_x(0)\doteq \xi^{-1}(0,\Xi)$ is an open set. As a consequence, $\Omega_y=\Omega_x\times\Xi$ is an open set.


Note that $\dot{\xi} =\frac{1}{p(t)}(\dot{e}-\xi(t)\dot{p})$. We have that $p(t)$, $e(t)$, $\dot{p}$ are continuous. Moreover, we have that $f$ and $g$ are Lipschitz. Thus we have that the dynamics $F(t,y)$ locally Lipschitz on $y$ and continuous on $t$ for any given $y$. Note that $\Omega_y$ is non-empty and open. Then by Lemma \ref{lemma:maximal sol}, we have that there exists a maximal solution $y=[x^\top,\xi]^\top$ such that $x(t)\in\Omega_x(0)$ and $\xi(t)\in\Xi$ for all $t\in[0,\tau_{\max})$.  
\end{proof}



% Denote the prescribed time for the system to return to $\mathcal{C}$ as $T$. We transform the finite time $T$ to coordinate $\mathbb{R}_{\geq 0}$ as
% \begin{equation}
%     \theta(s)=t,
% \end{equation}
% where $\theta:\mathbb{R}_{\geq 0}\rightarrow[0,T]$ is the transformation. Here $\theta(s)$ is defined as
% \begin{equation}
%     \theta(s)=T\left(1-\exp\left(-\frac{s}{T}\right)\right).
% \end{equation}

% We then convert Eqn. \eqref{eq:remaining budget time domain} into the domain of $\mathbb{R}_{\geq 0}$ as
% \begin{subequations}\label{eq:remaining budget s domain}
% \begin{align}
%     e(s) &= cB - J(\theta(s),x)\\
%     \xi(s) &= \frac{e(\theta(s))}{p(\theta(s))}\\
%     \epsilon(s) & = S(\xi(\theta(s)))=\ln\left(\frac{\xi(\theta(s))}{1-\xi(\theta(s))}\right)
% \end{align}
% \end{subequations}
% We now have the following dynamics:
% \begin{subequations}\label{eq:remaining budget s domain}
% \begin{align}
%     e'(s) &=-\frac{\partial J}{\partial x}\dot{x}\theta'(s)\\
%     \xi'(s) &= \frac{\dot{e}(\theta(s))p(\theta(s))-e(\theta(s))\dot{p}(\theta(s))}{p(\theta(s))^2}\theta'(s)\\
%     \epsilon'(s) & = \frac{1}{\xi(\theta(s))(1-\xi(\theta(s)))}\dot{\xi}(\theta(s))\theta'(s)
% \end{align}
% \end{subequations}
% In addition, the system dynamics is rewritten as
% \begin{equation}
%     x'(s) = (f(x)+g(x)u)\theta'(s).
% \end{equation}



\begin{proposition}\label{prop:control law}
Assume that the initial state of the normal state satisfies $\xi(t,x)\in(0,1)$. The control law
\begin{multline}\label{eq:control law}
    u(t,x) =\\
    \frac{-\frac{\partial J}{\partial x}f(x) - \xi \dot{p}+\epsilon\sqrt{(\frac{\partial J}{\partial x}f(x))^2+((\frac{\partial J}{\partial x}g(x))(\frac{\partial J}{\partial x}g(x))^\top)^2}}{(\frac{\partial J}{\partial x}g(x))(\frac{\partial J}{\partial x}g(x))^\top}(\frac{\partial J}{\partial x}g(x))^\top
\end{multline}
renders that $\dot{V}\leq 0$ for $t\in[0,\tau_{\max})$, whre $V=\frac{1}{2}\epsilon^2$.
\end{proposition}
\begin{proof}
Define $V(\epsilon)=\frac{1}{2}\epsilon^2$. We then have that
\begin{align*}
    \dot{V}=&\epsilon\dot{\epsilon}\\
    =&\epsilon\frac{\dot{e}-\xi\dot{p}}{p\xi(1-\xi)}\\
    =&\frac{\epsilon}{p\xi(1-\xi)}\left(-\frac{\partial J}{\partial x}(f(x)+g(x)u)-\xi\dot{p}\right)
\end{align*}
Substitute control law \eqref{eq:control law} into $\dot{V}$, we have that
\begin{equation}
    \dot{V}=-\frac{\epsilon^2}{p\xi(1-\xi)}\sqrt{(\frac{\partial J}{\partial x}f(x))^2+((\frac{\partial J}{\partial x}g(x))(\frac{\partial J}{\partial x}g(x))^\top)^2}
\end{equation}
Note that $\frac{1}{\xi(1-\xi)}>0$ for all $\xi\in(0,1)$. Additionally, Lemma \ref{lemma:existence of maximal sol} indicates that $\xi\in(0,1)$ for all $t\in[0,\tau_{\max})$. Therefore, we have that $\dot{V}\leq 0$ for all $t\in[0,\tau_{\max})$.
\end{proof}

\begin{corollary}
The control law \eqref{eq:control law} is continuous and bounded.
\end{corollary}
\begin{proof}
The corollary follows from the Lipschitz continuities and boundedness of $f$, $g$, $J$, and $\epsilon$.
\end{proof}

\begin{lemma}
Let $\tau_{\max}$ be as defined in Lemma \ref{lemma:existence of maximal sol} and the control law be given as in Proposition \ref{prop:control law}. Then $\tau_{\max}=\infty$.
\end{lemma}
\begin{proof}
We prove the lemma by contradiction. Suppose $\tau_{\max}<\infty$. By Proposition \ref{prop:control law}, we have that $|\epsilon|$ is upper and lower bounded. Let $\epsilon_{LB}$ and $\epsilon_{UB}$ be the lower and upper bounds of $\epsilon$, respectively. We then have that $\xi\in \Xi$ since transformation $S$ admits an inverse, yielding $\xi\in[\xi_{LB},\xi_{UB}]\subset(0,1)$ for some $\xi_{LB},\xi_{UB}\in(0,1)$ and $\xi_{LB}\leq\xi_{UB}$. Therefore, $\xi$ belongs to a compact set $[\xi_{LB},\xi_{UB}]$. By the definitions of $\xi$ and $p$, we have that $e(t)$ belongs to a compact set $\mathcal{E}$ as well. As a consequence, we have that $e^{-1}(\mathcal{E})=\{x:e(t,x)\in\mathcal{E}\}$ is closed. By Lemma \ref{lemma:infinity}, we have that when $y$ evolves in a compact set and $\tau_{\max}<\infty$, then there exists some $t$ such that $y(t)$ leaves the compact set. By contradiction, we have that $\tau_{\max}=\infty$.
\end{proof}

\begin{theorem}
The control law \eqref{eq:control law} guarantees that budget constraint $cB-J(t,x)\in(0,p(t))$ for $t\geq 0$.
\end{theorem}
\begin{proof}
The theorem follows from the intermediate result of Lemma 4, i.e., $\xi\in(0,1)$, the fact that $p(t)\geq0$ for all $t$, and $\tau_{\max}=\infty$.
\end{proof}

In the following, we show that the system returns to the safety set by implementing the control law \eqref{eq:control law} by properly designing performance function $p(t)$. Note that we need to ensure $\xi\in(0,1)$. Thus we have that
\begin{equation}
    p(0)>e(0).%\quad p_\infty\in(0,\inf_{x\notin\mathcal{C}}q(x)h(x)^2).
\end{equation}

\begin{lemma}
By implementing the control law \eqref{eq:control law}, the system can only leave the safety set $\mathcal{C}$ for finite time.
\end{lemma}
\begin{proof}
Note that $0<cB-J(t,x)$ is satisfied for all $t\geq 0$. If the lemma does not hold, we have that $0<cB-J(t,x)$ will be violated since there must exists some time $t$ such that $cB-J(t,x)<0$.
\end{proof}


==> formulation.tex <==
\section{System Model and Problem Formulation} \label{sec:system model}


We consider a cyber-physical system (CPS) consisting of a cyber subsystem and a physical subsystem. The physical subsystem models a plant that evolves following Eqn. \eqref{eq:dynamics},
where $x_t\in\mathbb{R}^n$ is the system state, $u_t\in\mathcal{U}\subset\mathbb{R}^m$ is the control input computed by the cyber subsystem. We also assume that $\mathcal{U}=\prod_{i=1}^m[u_{i,min},u_{i,max}]$ with $u_{i,min}<u_{i,max}$.

The physical plant is normally recommended to be operated within a certain range $\mathcal{C}\subset\mathbb{R}^n$ defined as $\mathcal{C} = \{x:h(x)\geq 0\}$, where $h:\mathbb{R}^n\rightarrow\mathbb{R}$ is a continuously differentiable function. In this paper, we assume that set $\mathcal{C}$ is compact.

The cyber subsystem interacts with the physical subsystem following functioning cycles. In each functioning cycle, the cyber subsystem reads the measurements from the sensors, calculates the output, and writes the signal to the actuator of the plant. In the remainder of this paper, we refer to a functioning cycle as epoch, and we assume that the sensors can directly measure the physical state $x$. Given the system state $x$, the cyber subsystem computes the actuator signal $u$ following a policy $\tau:\mathcal{X}\rightarrow\mathcal{U}$. Although the physical plant evolves in continuous time, the cyber system reads the sensor measurements and updates the actuator signal in a digital fashion. We denote the length of each epoch as $\delta>0$. Then the cyber system measures $x_{k\delta}$ and updates the actuator signal $u_{k\delta}=\mu(x_{k\delta})$ for each $k=0,1,\ldots$. The actuator signal remains constant during each epoch.

The CPS is subject to malicious attack initiated by an intelligent adversary. The adversary aims at destabilizing the physical plant to damage it. The adversary can exploit the vulnerabilities in the cyber subsystem and intrude into the system. Once the adversary intrudes successfully, it gains access to the software, actuators, and other peripherals. As a consequence, the actuator signal is corrupted by the adversary and deviates from the desired control policy $\mu(\cdot)$.

Due to the malicious attack, the physical plant may have to be temporarily operated outside $\mathcal{C}$. To avoid causing irreversible damage to the plant, we need to minimize the amount of time that the CPS is operated outside $\mathcal{C}$ or minimize the distance that the physical state $x$ deviates from $\mathcal{C}$. We capture the instantaneous damage incurred by the plant when operated outside $\mathcal{C}$ as a cost $L:\mathbb{R}\rightarrow\mathbb{R}$, defined as 
\begin{equation}\label{eq:cost}
    L(h(x)) = \begin{cases}
    L_1(-h(x)),&\mbox{ if }h(x)< 0\\
    0,&\mbox{ if }h(x)\geq 0
    \end{cases}
\end{equation}
where $L_1:\mathbb{R}^+\rightarrow\mathbb{R}_{\geq 0}$ is a monotone non-decreasing function. When $L_1(-h(x))$ is chosen as $L_1(-h(x))=1$, then we can use $\int_{t}L(x)\dd t$ to capture the amount of time such that $x_t\notin\mathcal{C}$. When $L_1(-h(x))=-h(x)$ for all $x\notin\mathcal{C}$, then Eqn. \eqref{eq:cost} models the deviation of the physical plant from the boundary of $\mathcal{C}$. We define the physical safety with respect to budget $B$ as follows.
\begin{definition}[Physical Safety with Respect to Budget $B$]\label{def:safety}
The physical plant is safe with respect to a budget $B$ if the following relation holds:
\begin{equation} 
    J=\int_{t=t_1}^{t_2}L(h(x_t))\dd t\leq B,~\forall 0\leq t_1< t_2 \label{budget}
\end{equation}
where $t_1\geq 0$ is the time instant when the adversary corrupts the cyber subsystem, and $t_2> t_1$ is the time instant at which the adversary corrupts the system again for the first time after the compromise at $t_1$.
\end{definition}

The budget $B$ sets an upper bound on the cost $J$ for a single successful attack by an adversary. Thus the Definition \ref{def:safety} indicates that the system is safe with respect to budget $B$ if the adversary can not cause more than $B$ cost to the system for each compromise effort. By setting $B=0$, we can recover the strict safety constraint defined over set $\mathcal{C}$, i.e., the physical plant leaving set $\mathcal{C}$ should be forbidden. 

We suppose that when the budget $B$ is violated (i.e. $J>B$), system reaches location $l=safety~violation$ implying irreversible damage to the plant. Here we are interested in obtaining a control policy such that system never reaches $l=safety~violation$ for an attack initiated at $l=normal$. Thus the problem we study here in this paper can be stated as:
\begin{problem} \label{prob1}
Synthesize a control policy for the CPS so that the physical subsystem is safe with respect to budget $B$.
\end{problem}


% In this paper, we investigate the following problem.
% \begin{problem}
% Develop a framework that unifies existing BFT++ based cyber resilience designs. Given the unified framework, synthesize a control policy $\mu$ such that $J(\mu,x_0)$ is minimized.
% \end{problem}

% Throughout this paper, we make the following assumptions.
% \begin{assumption}
% We assume that $(\frac{\partial J}{\partial x}g(x))(\frac{\partial J}{\partial x}g(x))^\top\neq 0$ for all $x\in\mathbb{R}^n$.
% \end{assumption}

==> framework.tex <==
\section{A Cyber Resilient Framework}\label{sec:framework}

In this section, we first summarize existing resilient designs. Then we present a framework that unifies the existing designs.

\subsection{Summary of the Existing Architectures} 


\emph{Cyber Resilient Design for CPS with Redundancy.} We first consider the class of CPS that has redundant resources such as controllers \cite{mertoguno2019physics,xu2017bunshin}. In this case, the system can deploy multiple replicas of the controller to disrupt the exploitation launched by the adversary. The deployed controllers are engineered to conduct the same mission with diversified mechanism such as software. Due to the diversification, the exploitation can only succeed for one controller while is to be less effective for the others. As a consequence, some deployed controllers will crash or the outputs from the controllers will diverge, indicating that an attack or fault has happened. Due to the periodicity of the functioning cycle, controller crash or output divergence may not happen instantaneously and incurs some delay. As a consequence, the adversary may own the cyber subsystem for a limited amount of time and arbitrarily manipulate the controller output. For instance, the controller crash can be delayed by at most $2$ epochs using the design proposed in \cite{mertoguno2019physics}. 

Once controller crash or output divergence occurs, the cyber subsystem transitions to the restoration mode to recover from the attack. The restoration leverages a delayed FIFO queue that is equipped to one controller which serves as the backup controller during restoration. The delayed FIFO queue stores the input in it, and feeds the data to the backup controller after a delay $D$. The delay $D$, which is also the length of the FIFO queue, is configured to be larger than the delayed incurred by the controller crash or output divergence, so that at least one uncorrupted input is stored in the FIFO queue. Using the delayed FIFO queue, we can recover the corrupted controllers using the backup. 

The system leverages physical inertia to avoid crash. In other words, the system is guaranteed to be safe if the controller is restored before utilizing the maximum tolerance provided by the physical inertia.

\emph{Cyber Resilient Design CPS without Redundancy.} We next consider the class of CPS that does not own redundant resources \cite{arroyo2019yolo}. Different from the aforementioned CPS with redundant resources, the CPS without redundancy cannot leverage diversified deployment to thwart exploitation from the adversary and recover from attack. Instead, the system conducts a system level reboot on the cyber side in a proactive or reactive manner. Proactive system restart uses a timer to trigger the system reboot. Reactive system restart uses controller crash to trigger system reboot. During the system reboot, the is no signal written to the actuator, leading to $u_t=0$.

\emph{Simplex Architecture.} The simplex architectures \cite{sha2001using,bak2009system,mohan2013s3a} consists a high performance controller that is vulnerable to random failures and a high assurance controller that is verifiable and fault-free. Once the high performance controller incurs failure, a decision module switches to the fault-free high assurance controller to control the system. In the meantime, the system can recover the failed high performance controller and switch to it later. We remark that the simplex architectures assume that the faulty behaviors only happens for some components in the system. When the system is under malicious attack, this assumption is violated since the adversary can proactively corrupt all components using the available resources to maximize its utility.


\begin{figure}
    \centering
    \includegraphics[scale=0.18]{diagram.png}
    \caption{We propose a hybrid system $H=(\mathcal{X},\mathcal{U},\mathcal{L},\mathcal{Y},\mathcal{Y}_0,Inv,\mathcal{F},\allowbreak \Sigma,\mathcal{E},\Phi)$ to capture simplex architecture (left part) and the cyber resilient architecture (right part). Each state $y=(x,(l_1,j))\in\mathcal{Y}$ of the hybrid system captures the continuous physical state $x\in\mathcal{X}$ and the discrete location $l=(l_1,j)\in\mathcal{L}$ including the system status $l_1$ and the epoch index $j$. Each circle in the figure represents a discrete location in $\mathcal{L}$, with the epoch indices being omitted. The arrows in the figure represent the transitions $\Sigma$ of hybrid system $H$. The transitions of form $(x,(l_1,j))$ are considered in hybrid system $H$, while not depicted in Fig. \ref{fig:unify framework} for compactness. Each transition $\sigma\in\Sigma$ is labeled using $e=(\gamma,e_2)\in\mathcal{E}$, where $\gamma$ denotes the event that triggers $\sigma$ and $e_2\in\mathbb{Z}_{\geq 0}$ represents the delay incurred by $\sigma$. Each transition from $y=(x,(l_1,j))$ to $y'=(x',l_1',j')$ is enabled when the event meets its label $\gamma$ and the corresponding clock constraint $\phi\in\Phi$ is satisfied. The clock constraint verifies the validity of $j,j'$ and $e_2$. We summarize the labels and clock constraints associated with each transition in Table \ref{table:transition}. The transition in red colors is triggered by external event, i.e., the adversarial cyber disruption. }
    \label{fig:unify framework}
\end{figure}

\begin{table*}[] 
    \centering
    \begin{tabular}{|c|c|c|c|c|}
    \hline
    Designs &Starting state $(x,(l_1,j))$  &  Target state $(x',(l_1',j'))$ & Label $e=(\gamma,e_2)$ & Clock constraint $\phi$\\
    \hline
    \hline
   \multirow{2}{*}{\shortstack[l]{Simplex \\architecture}} &  $(x,(normal,j))$    & $(x,(SC,j'))$ & $(Safety~controller~activated,e_2)$ & $ (j+e_2=j')\land (e_2=0)$\\
     \cline{2-5}
   &  $(x,(SC,j))$    & $(x,(normal,j'))$ & $(Safety~controller ~inactivated,e_2)$ & $(j+e_2=j')\land (e_2=0)$\\
     \hline
    \multirow{7}{*}{\shortstack[l]{Cyber\\ resilient\\ architectures}} &  $(x,(normal,j))$    & $(x',(corrupted,j'))$ & $(Adversarial~ cyber~ disruption,e_2)$ & $ (j+e_2=j')\land (e_2\geq 0)$\\
     \cline{2-5}
    &  $(x,(corrupted,j))$    & $(x',(restoration,j'))$ & $(Controller~crash,e_2)$ & $ (j+e_2=j')\land (e_2\leq N_1)$\\
    \cline{2-5}
     &  $(x,(restoration,j))$    & $(x',(normal,j'))$ & $(Controller~restored,e_2)$ & $ (j+e_2=j')\land (e_2\leq N_2)$\\
      \cline{2-5}
     &  $(x,(normal,j))$    & $(x',(R\&I,j'))$ & $(Timer,e_2)$ & $ (j+e_2=j')\land (e_2=N_5)$\\
     \cline{2-5}
     &  $(x,(corrupted,j))$    & $(x',(R\&I,j'))$ & $(Controller~crash\lor Timer,e_2)$ & $ (j+e_2=j')\land (e_2\leq N_3)$\\
     \cline{2-5}
     &  $(x,(R\&I,j))$    & $(x',(normal,j'))$ & $(Initialization~done,e_2)$ & $ (j+e_2=j')\land (e_2\geq N_4)$\\
     \cline{2-5}
     &  $(x,(\cdot,j))$    & $(x',(safety~violation,j'))$ & $(Maximum ~inertia ~tolerance,e_2)$ & $ (j+e_2=j')\land (e_2\geq \Delta(x))$\\
     \hline
    \end{tabular}
    \caption{This table shows the transitions with their corresponding labels and clock constraints. The second and third columns give the starting and end states of a transition, respectively. The fourth column presents the label $e=(\gamma,e_2)$ associated with the transition $\sigma=((x,(l_1,j)),(x',(l_1',j')))$. The trigger event of the transition is denoted as $\gamma$, and the delay incurred by the transition is denoted using $e_2\in\mathbb{Z}_{\geq 0}$. The fifth column gives the clock constraint $\phi$ that needs to be satisfied by the transition $\sigma$ and the delay $e_2$. Parameters $N_1,N_2,N_3,N_4$, and $N_5$ are determined by the architecture design. Parameter $\Delta(x)$ captures the maximum tolerance provided by the physical inertia.}
    \label{table:transition}
\end{table*}

\subsection{Our Proposed Framework}

In this subsection, we present a hybrid system $H=(\mathcal{X},\mathcal{U},\mathcal{L},\mathcal{Y},\mathcal{Y}_0,Inv,\mathcal{F},\allowbreak \Sigma,\mathcal{E},\Phi)$, as shown in Fig. \ref{fig:unify framework}, to model the aforementioned architectures, where
\begin{itemize}
    \item $\mathcal{X}\subseteq\mathbb{R}^{n}$ is the continuous state space modeling the states of the physical subsystem.
    \item $\mathcal{U}\subseteq\mathbb{R}^m$ is the set of admissible control inputs of the physical subsystem.
    \item $\mathcal{L}=\{normal, R\& I, SC, restoration,\allowbreak corrupted, \allowbreak safety~violation\}\times\mathbb{Z}_{\geq 0}$ is a finite set of discrete locations\footnote{In the remainder of this paper, we denote $l=reboot\&initialization$ as $l=R\&I$ and denote $l=safety~controller~driven$ as $l=SC$ for simplicity.}, where the former models the status of the system, and the latter gives the current epoch index. 
    \item $\mathcal{Y}=\mathcal{X}\times\mathcal{L}$ is the state space of hybrid system $H$, and $\mathcal{Y}_0\subseteq \mathcal{Y}$ is the set of initial states.
    \item $Inv:\mathcal{L}\rightarrow 2^\mathcal{X}$ is the invariant that maps from the set of locations to the power set of $\mathcal{X}$. That is, $Inv(l)\subseteq\mathcal{X}$ specifies the set of possible continuous states when the system is at location $l$.
    \item $\mathcal{F}$ is the set of vector fields. For each $F\in\mathcal{F}$, the continuous system state evolves as $\dot{x}=F(x,u,l)$, where $F:\mathcal{X}\times\mathcal{U}\times\mathcal{L}\rightarrow\mathcal{X}$ and $\dot{x}$ is the time derivative of continuous state $x$.
    \item $\Sigma\subseteq \mathcal{Y}\times \mathcal{Y}$ is the set of transitions between the states of the hybrid system. A transition $\sigma=((x,l),(x',l'))$ models that the hybrid state transitions from $(x,l)$ to $(x',l')$.
    \item $\mathcal{E}=\Gamma\cup\mathbb{Z}_{\geq 0}$ is a set of labels, where $\Gamma$ is the finite alphabet set and $\mathbb{R}_{\geq 0}$ is the continuous label associated with time. Each $\gamma\in\Gamma$ is labeled on some transition $\sigma\in \Sigma$ indicating the events that triggers the transition. 
    \item $\Phi$ is a set of clock constraints, with each $\phi\in\Phi$ being defined as $\phi: \Sigma\times \mathbb{Z}_{\geq 0}\rightarrow\{0,1\}$. Function $\phi$ maps the time elapsed in each discrete location and the epoch indices to the binary set $\{0,1\}$, indicating if the transition is enabled or not.
\end{itemize}
In Fig. \ref{fig:unify framework}, we only label the first element of each location $l=(l_1,j)$, where $l_1\in\{normal, R\& I, SC, restoration,\allowbreak corrupted, \allowbreak safety~violation\}$ and $j\in\mathbb{Z}_{\geq 0}$. The epoch index $j$ is omitted in Fig. \ref{fig:unify framework}. The set of vector fields $\mathcal{F}$ captures the dynamics at each discrete location. For instance, when $l=(normal,j)$, we have that $\dot{x}=F(x,u,l)=f(x)+g(x)u$ for all $j\in\mathbb{Z}_{\geq 0}$, where $u\in\mathcal{U}$ is the control input. 

We label each transition $\sigma=((x,l),(x',l'))\in\Sigma$ using $e=(\gamma,e_2)\in\mathcal{E}$. The detailed label associated with each transition can be found in Table \ref{table:transition}. Here we use $\gamma$ to represent the event that triggers the transition. For instance, the transition from $(x,(normal,j))$ to $(x',(corrupted,j'))$ is triggered by the adversarial cyber disruption, whereas the transition from $(x,(corrupted,j))$ to $(x',(restoration,j'))$ is triggered by controller crash. The element $e_2\in\mathbb{Z}_{\geq 0}$ denotes the number of epochs elapsed in location $l$ before the occurrence of transition $\sigma=((x,l),(x',l'))$. When $e_2=0$, it indicates that the transition occurs instantaneously. When $e_2>0$, it implies that the transition incurs some delay $e_2$, which is determined by the architecture. For example, the transition from $(x,(corrupted,j))$ to $(x',(restoration,j'))$ incurs a delay by at most $N_1$ epochs. In \cite{mertoguno2019physics}, the worst-case delay is $N_1=2$.

A transition in hybrid system $H$ is enabled if and only if a clock constraint $\phi$ associated with the transition is satisfied. Consider a transition $\sigma=((x,(l_1,j)),(x',(l_1',j')))$ labeled with $e=(\gamma,e_2)$. A clock constraint $\phi$ verifies if $j$, $j'$, and $e_2$ satisfies whether (i) $j+e_2=j'$, and (ii) $e_2$ satisfies the condition determined by the architecture design. Condition (i) enables system $H$ always track the correct epoch index. Condition (ii) requires the transition to satisfy the architecture design. For example, the worst-case delay $e_2$ from $(x,(corrupted,j))$ to $(x',(restoration,j'))$ in \cite{mertoguno2019physics} is $N_1=2$. Then we need $e_2$ to satisfy $e_2\leq N_1$.

The transitions that end at $l_1=safety~violation$ are triggered by event $\gamma=Maximum~inertial~tolerance$, indicating that the physical subsystem has not received the correct input and has utilized all tolerance provided by physical inertia. In this case, safety violation becomes inevitable, and the system cannot recover after safety violation (captured via the self-loop in Fig. \ref{fig:unify framework}). We capture the maximum tolerance provided by the inertia using the delay $e_2$ labeled on the transitions. Note that the tolerance depends on the physical system state $x$, and we denote the maximum delay as $\Delta(x)$. 

We remark that for each $l_1$, we do not depict the transitions $(x,(l_1,j))$ to $(x,(l_1,j+1))$ for compactness of the figure. These are the transitions that do not cause any system status jump, and only tracks the evolution of epoch indices. However, we would like to emphasize that these transitions exist in practice and are captured by hybrid system $H$. 

We finally define a guard set $\mathcal{G}(l,l')$ as $\mathcal{G}(l,l')=\{x \in \mathcal{X}: ((x,l),(x,l')) \in \Sigma \}$ which models the set of continuous states starting from which the system can transition from location $l$ to $l'$ under the conditions labeled with the transition. When the context is clear, we use $l=normal$ to represent the location $l=(normal,j)$ for some non-negative integer $j$.

% The hybrid system captures the continuous physical state transition following dynamics \eqref{eq:dynamics} and the discrete cyber status transition. When there exists no adversary or fault in the system, the discrete location set $\mathcal{L}=\{normal\}$ becomes a singleton, and the hybrid system reduces to a continuous system controlled by a cyber subsystem that is always in normal status. 

% When there exists a malicious adversary or some components are subject to faults, the proposed hybrid system captures the existing defending/recovery strategies such as \cite{mertoguno2019physics,arroyo2019yolo}. When the CPS has redundancy, then the cyber subsystem can be restored (captured via discrete location $l=restoration$). While for the CPS without redundancy, the cyber subsystem needs to reboot and be reinitialized (captured via discrete location $l=R\&I$).

% The lower part of Fig. \ref{fig:unify framework} models BFT++. BFT++ only triggers controller crash once the adversary exploits the vulnerabilities of the system. In this case, the only controller that is still online is the one that is owned by the adversary, whose output cannot be trusted. We denote this status as vulnerable in Fig. \ref{fig:unify framework}. As a response, the crashed controllers switch to restoration mode to recover from the attack (as labeled in the purple box). Since controllers may not crash immediately after exploitation, we model the controller crash delay on the transitions from vulnerable to restore. During the controller restoration, the controller output is set as the one obtained from the delay FIFO queue. After the controller restoration, the system returns back to the normal operation.

% The upper part of Fig. \ref{fig:unify framework} captures YOLO \cite{arroyo2019yolo}. The controller switches to initialization either due to timer setup or controller crash. During the controller initialization, the controller cannot produce any output. After the controller initialization, the controller is back online, making the system to be operated in the normal mode.

==> framework_v2.tex <==
\section{Our Proposed Cyber Resilient Framework}\label{sec:framework}

In this section, we first briefly review the cyber resilient architectures \cite{mertoguno2019physics,arroyo2019yolo,xu2017bunshin}. Next we construct a hybrid system that can be used to model CPS adopting these different architectures, which will be used later to solve Problem \ref{prob1}. The simplex architecture reviewed in Section \ref{sec:related} is also incorporated in our framework for completeness. 

\subsection{Review of Cyber Resilient Architectures}\label{sec:architecture} 

In this subsection, we review the family of BFT++ \cite{mertoguno2019physics,arroyo2019yolo,xu2017bunshin} by dividing out discussion on CPS with redundant controllers and CPS without redundant controllers.

When CPS has redundant controllers \cite{mertoguno2019physics,xu2017bunshin}, the crashed ones and corrupted ones are recovered using the state of a backup controller that is appropriately delayed using a buffer. To guarantee the safety of the physical subsystem, the system needs to satisfy the following conditions:
\begin{itemize}
    \item[C1] the controllers should crash before the backup controller gets corrupted by the malicious input injected into the buffer by the adversary;
    \item[C2] the resilience provided by the physical subsystem should tolerate the cyber recovery latency.
\end{itemize}

For CPS without redundant controllers, the system proactively restarts to recover from attack \cite{arroyo2019yolo}. It is proved that if the following conditions hold:
\begin{itemize}
    \item[C3] the controller restart frequency is upper bounded;
    \item[C4] the controller availability is lower bounded  by some threshold (determined using the transfer function),
\end{itemize}
then the physical subsystem is safe.  

In the next subsection, we will show how conditions C1-C4 can be captured using our proposed framework.


% We first consider the class of CPS that has redundant resources such as controllers \cite{mertoguno2019physics,xu2017bunshin}. The CPS deploy multiple replicas of the controller to disrupt the exploitation launched by the adversary. The deployed controllers are engineered to conduct the same mission with diversified mechanism such as software. Due to the diversification, the exploitation can only succeed for one controller while is to be less effective for the others. As a consequence, some deployed controllers will crash or the outputs from the controllers will diverge, indicating that an attack or fault has happened. Due to the periodicity of the functioning cycle, controller crash or output divergence may not happen instantaneously and incurs some delay. As a consequence, the adversary may own the cyber subsystem for a limited amount of time and arbitrarily manipulate the controller output. For instance, the controller crash can be delayed by at most $2$ epochs using the design proposed in \cite{mertoguno2019physics}. Once controller crash or output divergence occurs, the cyber subsystem restores the owned and crashed controllers from a fresh state or to a known good state via a buffer implemented to one of replicas.


% We next consider the class of CPS without redundancies \cite{arroyo2019yolo,abdi2018guaranteed}. The CPS without redundancies cannot leverage diversified deployment to thwart exploitation from the adversary. Instead, the system conducts a system level reboot on the cyber side in a proactive or reactive manner to recover the system. Proactive system restart uses a timer to trigger the system reboot. Reactive system restart uses controller crash to trigger system reboot. During the system reboot, the is no signal written to the actuator, leading to $u_t=0$. 

% While the crash delay, restoration time, and system reboot time depend on cyber subsystem properties and the resilient design, the tolerance provided of the physical subsystem varies for different systems. Thus the cyber resilient designs and control policies need to be carefully tailored to guarantee safety of the physical subsystem. In the next subsection, we propose a framework with a set of tunable parameters that captures the existing fault tolerant and cyber resilient architectures. 

\begin{figure}
    \centering
    \includegraphics[scale=0.185]{diagram.png}
    \caption{Hybrid system $H=(\mathcal{X},\mathcal{U},\mathcal{L},\mathcal{Y},\mathcal{Y}_0,Inv,\mathcal{F},\allowbreak \Sigma,\allowbreak\mathcal{E},\allowbreak\Phi)$ captures the simplex architecture (left part) and the cyber resilient architecture (right part). Each state $y=(x,(l_1,j))\in\mathcal{Y}$ of the hybrid system captures the continuous physical state $x\in\mathcal{X}$ and the discrete location $l=(l_1,j)\in\mathcal{L}$ including the system status $l_1$ and the epoch index $j$. Each circle in the figure represents a discrete location in $\mathcal{L}$, with the epoch indices being omitted. The arrows in the figure represent the transitions $\Sigma$ of hybrid system $H$. Each transition is labeled using $e\in\mathcal{E}$, and is enabled when the corresponding clock constraint $\phi\in\Phi$ is satisfied. The labels and clock constraints associated with each transition are given in Table \ref{table:transition}. The transition in red color is triggered by external event, i.e., the adversarial cyber disruption. }
    \label{fig:unify framework}
\end{figure}

\begin{table*}[] 
    \centering
    \begin{tabular}{|m{13mm}|c|c|c|m{33mm}|}
    \hline
    Designs &Starting state $(x,(l_1,j))$  &  Target state $(x',(l_1',j'))$ & Label $e=(\gamma,e_2)$ & Clock constraint $\phi$\\
    \hline
    \hline
   \multirow{2}{*}{\shortstack[l]{Simplex \\architecture}} &  $(x,(normal,j))$    & $(x,(SC,j'))$ & $(Safety~controller~activated,e_2)$ & $ (j+e_2=j')\land (e_2=0)$\\
     \cline{2-5}
   &  $(x,(SC,j))$    & $(x,(normal,j'))$ & $(Safety~controller ~inactivated,e_2)$ & $(j+e_2=j')\land (e_2=0)$\\
     \hline
    \multirow{7}{*}{\shortstack[l]{the Family\\of BFT++}} &  $(x,(normal,j))$    & $(x',(corrupted,j'))$ & $(Adversarial~ cyber~ disruption,e_2)$ & $ (j+e_2=j')\land (e_2\geq 0)$\\
     \cline{2-5}
    &  $(x,(corrupted,j))$    & $(x',(restoration,j'))$ & $(Controller~crash,e_2)$ & $ (j+e_2=j')\land (e_2\leq N_1)$\\
    \cline{2-5}
     &  $(x,(restoration,j))$    & $(x',(normal,j'))$ & $(Controller~restored,e_2)$ & $ (j+e_2=j')\land (e_2\leq N_2)$\\
      \cline{2-5}
     &  $(x,(normal,j))$    & $(x',(R\&I,j'))$ & $(Timer,e_2)$ & $ (j+e_2=j')\land (e_2=N_5)$\\
     \cline{2-5}
     &  $(x,(corrupted,j))$    & $(x',(R\&I,j'))$ & $(Controller~crash\lor Timer,e_2)$ & $ (j+e_2=j')\land (e_2\leq N_3)$\\
     \cline{2-5}
     &  $(x,(R\&I,j))$    & $(x',(normal,j'))$ & $(Initialization~done,e_2)$ & $ (j+e_2=j')\land (e_2\geq N_4)$\\
     \cline{2-5}
     &  $(x,(\cdot,j))$    & $(x',(safety~violation,j'))$ & $(Maximum ~tolerance,e_2)$ & $ (j+e_2=j')\land (e_2\geq \Delta(x))$\\
     \hline
    \end{tabular}
    \caption{This table shows the transitions with their corresponding labels and clock constraints. The second and third columns give the starting and end states of a transition, respectively. The fourth column presents the label $e=(\gamma,e_2)$ associated with the transition $\sigma=((x,(l_1,j)),(x',(l_1',j')))$. The trigger event of the transition is denoted as $\gamma$, and the time elapsed in $l_1$ is denoted using $e_2\in\mathbb{Z}_{\geq 0}$. The fifth column gives the clock constraint $\phi$ that needs to be satisfied by the transition $\sigma$ and parameter $e_2$. Parameters $N_1,N_2,N_3,N_4$, and $N_5$ are determined by the architecture design. Parameter $\Delta(x)$ captures the maximum tolerance provided by the physical subsystem.}
    \label{table:transition}
\end{table*}

\subsection{Our Proposed Framework}

In this subsection, we first construct a hybrid system to capture the CPS implementing the simplex or cyber resilient architectures introduced in Section \ref{sec:architecture}. We then formulate the problem of synthesizing a controller with safety guarantee. We construct a hybrid system $H=(\mathcal{X},\mathcal{U},\mathcal{L},\mathcal{Y},\mathcal{Y}_0,Inv,\mathcal{F},\allowbreak \Sigma,\mathcal{E},\Phi)$, as shown in Fig. \ref{fig:unify framework}, where
\begin{itemize}
    \item $\mathcal{X}\subseteq\mathbb{R}^{n}$ is the continuous state space modeling the states of the physical subsystem.
    \item $\mathcal{U}\subseteq\mathbb{R}^m$ is the set of admissible control inputs of the physical subsystem.
    \item $\mathcal{L}=\{normal, R\& I, SC, restoration,\allowbreak corrupted, \allowbreak safety~violation\}\times\mathbb{Z}_{\geq 0}$ is a set of discrete locations\footnote{Throughout this paper, we denote $l=reboot\&initialization$ as $l=R\&I$ and denote $l=safety~controller~driven$ as $l=SC$ for simplicity.}, with each location $l\in\mathcal{L}$ modeling the status of the system at each epoch index. 
    \item $\mathcal{Y}=\mathcal{X}\times\mathcal{L}$ is the state space of hybrid system $H$, and $\mathcal{Y}_0\subseteq \mathcal{Y}$ is the set of initial states.
    \item $Inv:\mathcal{L}\rightarrow 2^\mathcal{X}$ is the invariant that maps from the set of locations to the power set of $\mathcal{X}$. That is, $Inv(l)\subseteq\mathcal{X}$ specifies the set of possible continuous states when the system is at location $l$.
    \item $\mathcal{F}$ is the set of vector fields. For each $F\in\mathcal{F}$, the continuous system state evolves as $\dot{x}=F(x,u,l)$, where $F$ is jointly determined by the system dynamics and the status of the cyber subsystem, and $\dot{x}$ is the time derivative of continuous state $x$.
    %\mathcal{X}\times\mathcal{U}\times\mathcal{L}\rightarrow\mathcal{X}
    \item $\Sigma\subseteq \mathcal{Y}\times \mathcal{Y}$ is the set of transitions between the states of the hybrid system. A transition $\sigma=((x,l),(x',l'))$ models the state transition from $(x,l)$ to $(x',l')$.
    \item $\mathcal{E}=\Gamma\cup\mathbb{Z}_{\geq 0}$ is a set of labels, where $\Gamma$ is the finite alphabet set. Each $\gamma\in\Gamma$ is labeled on some transition $\sigma\in \Sigma$ indicating the events that triggers the transition.
    \item $\Phi$ is a set of clock constraints, with each $\phi\in\Phi$ being defined as $\phi: \Sigma\times \mathbb{Z}_{\geq 0}\rightarrow\{0,1\}$. Function $\phi$ maps the time elapsed in each discrete location labeled on each transition to the binary set $\{0,1\}$, indicating if the transition is enabled or not.
\end{itemize}
In Fig. \ref{fig:unify framework}, we only label the first element of each location $l=(l_1,j)$, where $l_1\in\{normal, R\& I, SC, restoration,\allowbreak corrupted, \allowbreak safety~violation\}$, and the epoch index $j\in\mathbb{Z}_{\geq 0}$ is omitted. In the remainder of this paper, we refer to $l_1$ as the location of $H$ when the context is clear. The set of vector fields $\mathcal{F}$ captures the dynamics at each discrete location. For instance, when $l=(R\&I,j)$, we have that $\dot{x}=F(x,u,l)=f(x)$ for all $j\in\mathbb{Z}_{\geq 0}$ since $u_t=0$.

We label each transition $\sigma=((x,l),(x',l'))\in\Sigma$ using $e=(\gamma,e_2)\in\mathcal{E}$. The detailed label associated with each transition can be found in Table \ref{table:transition}. Here we use $\gamma$ to represent the event that triggers the transition. For instance, the transition from $(x,(normal,j))$ to $(x',(corrupted,j'))$ is triggered by the adversarial cyber disruption, whereas the transition from $(x,(corrupted,j))$ to $(x',(restoration,j'))$ is triggered by controller crash. The element $e_2\in\mathbb{Z}_{\geq 0}$ denotes the number of epochs elapsed in location $l$ before the occurrence of transition $\sigma=((x,l),(x',l'))$. For example, at most $N_1$ epochs elapse at location $corrupted$ before the transition from $(x,(corrupted,j))$ to $(x',(restoration,j'))$ occurs. In \cite{mertoguno2019physics}, the worst-case delay is $N_1=2$. When $e_2=0$, it indicates that the transition occurs instantaneously. 

A transition in hybrid system $H$ is enabled if and only if a clock constraint $\phi$ associated with the transition is satisfied. Consider a transition $\sigma=((x,(l_1,j)),(x',(l_1',j')))$ labeled with $e=(\gamma,e_2)$. A clock constraint $\phi$ verifies if $j$, $j'$, and $e_2$ satisfies $j+e_2=j'$ with $e_2$ being determined by the architecture design. The clock constraint enables hybrid system $H$ to always track the correct epoch index. 

%We remark that for each $l_1$, we do not depict the transitions $(x,(l_1,j))$ to $(x,(l_1,j+1))$ for compactness of the figure. These are the transitions that do not cause any system status jump, and only tracks the evolution of epoch indices. However, we would like to emphasize that these transitions exist in practice and are captured by hybrid system $H$. We also define a guard set $\mathcal{G}(l,l')$ as $\mathcal{G}(l,l')=\{x \in \mathcal{X}: ((x,l),(x,l')) \in \Sigma \}$ which models the set of continuous states starting from which the system can transition from location $l$ to $l'$ under the conditions labeled with the transition.

We remark that for each $l_1$, we do not depict the transitions $(x,(l_1,j))$ to $(x,(l_1,j+1))$ for compactness of the figure. These are the transitions that do not cause any system status jump, and only tracks the evolution of epoch indices. We also define a guard set $\mathcal{G}(l,l')$ as $\mathcal{G}(l,l')=\{x \in \mathcal{X}: ((x,l),(x,l')) \in \Sigma \}$ which models the set of continuous states starting from which the system can transition from location $l$ to $l'$ under the conditions labeled with the transition.

The transitions that end at $l_1=safety~violation$ are triggered by event $\gamma=Maximum~tolerance$, indicating that the physical subsystem has not received the correct input in time and has utilized all tolerance of disruption. In this case, safety violation $J>B$ becomes inevitable, and the system cannot recover after safety violation (captured via the self-loop in Fig. \ref{fig:unify framework}). We capture the maximum tolerance using $e_2$ labeled on the transitions. Note that the tolerance depends on the physical system state $x$, and we denote the maximum delay as $\Delta(x)$. 

We next show how to use hybrid system $H$ to encode conditions C1-C4 given in Section \ref{sec:architecture}. Condition C1 is encoded using transition the transition from $l_1=corrupted$ to $l_1'=restoration$ as $e_2\leq N_1$ as shown in Table \ref{table:transition}, where parameter $N_1$ captures the controller crash delay. Condition C2 is modeled by the transition from $l_1=restoration$ to $l_1=normal$ as $e_2\leq N_2\leq \Delta(x)$. Here $N_2$ models the recovery latency. As we will show in Section \ref{sec:analysis}, our framework recovers condition C3 by lower bounding the length of attack cycle $A$. Hybrid system $H$ models controller availability as $\frac{e_2}{T}$, where $e_2$ is the time elapsed in $l_1=normal$ and $T$ is the time between two consecutive restarts. When the system restart is triggered by the timer, $e_2=N_5-N_4$ and $T=N_5$.


We are now ready to translate problem \ref{prob1} using the context of hybrid system $H$ as follows:\\
\textbf{Restatement of Problem \ref{prob1}.} Given hybrid system $H$, synthesize a control policy $\mu:\mathcal{X}\rightarrow\mathcal{U}$ such that hybrid system $H$ never reaches location $l=safety~violation$.



% The hybrid system captures the continuous physical state transition following dynamics \eqref{eq:dynamics} and the discrete cyber status transition. When there exists no adversary or fault in the system, the discrete location set $\mathcal{L}=\{normal\}$ becomes a singleton, and the hybrid system reduces to a continuous system controlled by a cyber subsystem that is always in normal status. 

% When there exists a malicious adversary or some components are subject to faults, the proposed hybrid system captures the existing defending/recovery strategies such as \cite{mertoguno2019physics,arroyo2019yolo}. When the CPS has redundancy, then the cyber subsystem can be restored (captured via discrete location $l=restoration$). While for the CPS without redundancy, the cyber subsystem needs to reboot and be reinitialized (captured via discrete location $l=R\&I$).

% The lower part of Fig. \ref{fig:unify framework} models BFT++. BFT++ only triggers controller crash once the adversary exploits the vulnerabilities of the system. In this case, the only controller that is still online is the one that is owned by the adversary, whose output cannot be trusted. We denote this status as vulnerable in Fig. \ref{fig:unify framework}. As a response, the crashed controllers switch to restoration mode to recover from the attack (as labeled in the purple box). Since controllers may not crash immediately after exploitation, we model the controller crash delay on the transitions from vulnerable to restore. During the controller restoration, the controller output is set as the one obtained from the delay FIFO queue. After the controller restoration, the system returns back to the normal operation.

% The upper part of Fig. \ref{fig:unify framework} captures YOLO \cite{arroyo2019yolo}. The controller switches to initialization either due to timer setup or controller crash. During the controller initialization, the controller cannot produce any output. After the controller initialization, the controller is back online, making the system to be operated in the normal mode.

==> intro.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Introduction}\label{sec:intro}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Cyber-physical systems (CPS) has found wide range of applications in transportation, energy, health and critical infrastructures \cite{??}. However, CPS are subject to cyber attacks due to software vulnerabilities present in the cyber part which introduces additional safety threats for the physical plants besides faults and failures. These cyber attacks may lead to severe damage to the physical plants and harm to environments and humans \cite{??}. Though IT defense approaches can provide high level protection to CPS, still there is possibility of low-level attacks on bus or back plane of CPS. This has motivated recent research attention in resiliency of CPS with a focus on leveraging useful properties of the physical subsystem \cite{??}.

Recently proposed resilient CPS architectures take advantage of inertia of the physical plant as well as large difference between physical and cyber time scale. This allow physical plant to tolerate short term disruptions occurring from cyber side. Based on this idea few resilient architectures have been proposed for redundant systems implementing diversity and buffer in the replicas \cite{??}. Proactive or reactive restarts have been proposed for CPS without redundancy with the idea that during reboot/restart the inertia of physical subsystem maintains safety \cite{??}. Switching between controllers running in parallel has also been proposed to guard against faults and failures with the assumption that high assurance controller guarantees safety in presence of fault \cite{?}. However safety against adversarial attack is not guaranteed in this architecture \cite{?}. 

%However, how the timing parameters or the control policy should be selected for non-linear plant is still unaddressed. 

Though several resilient CPS architectures have already been deployed, however a comprehensive analysis and formal safety guarantee for different sort of cyber attacks are still missing in the current literature. Specifically, how much tolerance a physical plant is able to provide for malicious input or how the control policy can be obtained for a nonlinear sophisticated plant with safety guarantee are yet to be studied analytically. Motivated by this in our study we aim to develop an analytical framework that can be used to design control policy and verify safety of the state-of-the-art resilient architectures. We make the following specific contributions in this work:

\begin{itemize}
    \item We develop a cyber resilient framework that unifies existing resilient architectures proposed in \cite{??}. In our framework we present a hybrid model that captures different phases of operation of CPS in these multiple architectures allowing mathematical analysis. 
    \item We derive sufficient conditions for control policy that satisfy safety with respect to a specified budget using a control barrier function type approach. Our results apply to wide range of safety constraints including hard constraints on system trajectory. 
    \item We develop an algorithm based on quadratic programming that can compute our proposed control policy and associate parameters for polynomial systems. Given that feasible solution exits our algorithm can find the solution in finite number of iteration.
    \item  We validate our proposed approach using a case study on lateral control of Boeing 747. Our simulation show that control policy obtained by our algorithm satisfies given budget constraint.
    
\end{itemize}

%In this context our previous work only considered reactive restart-based approach and for hard safety constraint. In this work we develop a unified model which captures the state-of-the-art resilient architectures and an analytical framework to design control policy that maintain safety for given budget constraint. 

The reminder of the paper is organized as follows. Section \ref{sec:related} presents related work where Section \ref{sec:preli} presents preliminary background. Section \ref{sec:framework} presents the our proposed cyber resilient framework. Section \label{sec:system model} formulates the problem that we study here. The analysis of the proposed framework and our solution to the problem are presented in the Section \ref{sec:analysis}. Section \ref{sec:simulation} presents a case a study while conclusion is made in Section \ref{sec:conclusion}.

==> intro_v2.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Introduction}\label{sec:intro}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Cyber-physical systems (CPS) are subject to random failures and malicious cyber attacks, which have been reported in applications such as transportation \cite{Jeep} and power system \cite{case2016analysis}. The failures and attacks can potentially cause safety violation of the physical components, which will further lead to severe damage to the plants and harm to humans. 

% To this end, fault tolerant \cite{sha2001using} and resilient CPS architectures \cite{mertoguno2019physics,arroyo2019yolo,abdi2018guaranteed} have been proposed, which take advantage of the inertia of the physical plant as well as the difference between physical and cyber time scales. These architectures rely on the observation that physical plants can tolerate cyber disruptions for a limited time due to inertia. During the time period driven by the inertia, the architecture can recover the system without human intervention.

To this end, fault tolerant \cite{sha2001using} and resilient CPS architectures \cite{mertoguno2019physics,arroyo2019yolo,abdi2018guaranteed} have been proposed. Fault tolerant architectures instantaneously invoke safety controller which is assumed to be fault-free to guarantee system safety once the system incurs faults in other components \cite{sha2001using}. Cyber resilient architectures \cite{mertoguno2019physics,arroyo2019yolo,abdi2018guaranteed} leverage the observation that the physical subsystem has natural resilience since its states usually do not change abruptly. Using this observation and the difference between the time scales in cyber and physical subsystems, cyber resilient architectures can tolerate short-term disruptions and recover the compromised cyber subsystem.

% which take advantage of the inertia of the physical plant as well as the difference between physical and cyber time scales. These architectures rely on the observation that physical plants can tolerate cyber disruptions for a limited time due to inertia. During the time period driven by the inertia, the architecture can recover the system without human intervention.

Since CPS vary from each other in multiple aspects such as the frequency of the cyber subsystem and the dynamics of the physical plant, the control synthesis for CPS implementing different architectures differs. As a consequence, engineers need to be knowledgeable about the system to synthesize control policies with formal safety guarantee. For instance, a control policy with safety guarantee can be synthesized using real-time computation of reachable states and considering the linearized system model \cite{abdi2018guaranteed}. However an analytic approach that applies to a general nonlinear system or legacy system with limited capability is of further interest. In addition, a safe control policy committed by a system implementing one architecture may not even work as expected for other systems or for the same system in the future. The reason is that CPS evolve rapidly over time as new subsystems comprising the existing one to satisfy increasingly complex and emerging requirements. To this end, we need a comprehensive framework that is applicable to CPS implementing different architectures to provide formal safety guarantee. However, to the best of our knowledge, such a framework has been less studied.

%e.g., some new component is later introduced into the system making the linear system dynamics to nonlinear.

% While CPS vary from each other in multiple aspects such as the frequency of the cyber subsystem and the dynamics of the physical plant, the existing architectures are system dependent. Thus a successful architecture implemented for one system may not work as expected for other systems or for the same system in the future, e.g., some new component is later introduced into the system and changes the system dynamics. To this end, we need a comprehensive framework that is applicable to CPS with different settings to provide formal safety guarantee, which has been less studied.

In this paper, we develop an analytical framework that can be used to design control policy for CPS with different settings. Our proposed framework captures the state-of-the-art architectures \cite{sha2001using,mertoguno2019physics,arroyo2019yolo}. The control synthesis conducted using our proposed framework provides formal safety guarantee and can be computed offline using the system dynamics. As our approach is not limited to specific architecture, thereby when the system evolve over time or switch to different fault tolerant or cyber resilient architectures, the control policy can be easily updated by tuning a set of parameters without weakening the safety guarantee. In this paper we make the following specific contributions:
\begin{itemize}
    \item We develop a framework that unifies the existing fault tolerant and cyber resilient architectures. We construct a hybrid system to model CPS implementing different architectures.
    \item We derive the sufficient conditions for a control policy to satisfy safety with respect to a specified budget using a control barrier function (CBF)-based approach. Our results recovers strict safety constraint as a special case.
    \item We develop an algorithm to compute a control policy that satisfies our derived conditions. Our proposed algorithm converges to a feasible solution, given its existence, within finite number of iterations.
    \item  We validate our proposed approach using a case study on lateral control of Boeing 747. We show that our proposed approach guarantees the safety of Boeing 747 with respect to the given budget constraint.
\end{itemize}

%In this context our previous work only considered reactive restart-based approach and for hard safety constraint. In this work we develop a unified model which captures the state-of-the-art resilient architectures and an analytical framework to design control policy that maintain safety for given budget constraint. 

The reminder of the paper is organized as follows. Section \ref{sec:related} presents related work. Section \ref{sec:preli} presents preliminary background. Section \ref{sec:system model} introduces the CPS model and presents the problem statement. Section \ref{sec:framework} gives our proposed framework. Section \ref{sec:analysis} presents our proposed solution approach. Section \ref{sec:simulation} contains a case a study and Section \ref{sec:conclusion} concludes the paper.

==> intro_v3.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Introduction}\label{sec:intro}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Cyber-physical systems (CPS) are subject to random failures and malicious cyber attacks, which have been reported in applications such as transportation \cite{Jeep} and power system \cite{case2016analysis}. The failures and attacks can potentially cause safety violation of the physical components, which will further lead to severe damage to the plants and harm to humans. 

To address random failures, the simplex architecture \cite{sha2001using} and its variants \cite{bak2009system,mohan2013s3a} are widely adopted. These architectures ensure safety by constraining the system states within an envelope using a safety controller. This safety controller is assumed to be fault-free and is usually chosen from some well-established classical controllers. However an adversary may corrupt the safety controller through malicious attack and violate safety.

To provide safety and resiliency against adversary, Byzantine fault tolerant++ (BFT++) architecture \cite{mertoguno2019physics} is proposed and already found application to different CPS \cite{xu2017bunshin,arroyo2019yolo}. BFT++ and its variations \cite{mertoguno2019physics,xu2017bunshin,arroyo2019yolo} utilize the fact that the physical subsystem follows the law of physics and has natural resilience against limited cyber disruptions due to difference of time scales in cyber and physical subsystems. 



However, due to disparity in implementation and timing behaviours among these variants, analysis undertaken for these variations are quite distinct and sometimes informal or restrictive. As example, vanilla BFT++ relies on fast and guaranteed reconstruction of corrupted controllers from a redundant controller with appropriate delay to ensure safety \cite{mertoguno2019physics} whereas \cite{arroyo2019yolo} (referred as YOLO) guarantees safety through restart and appropriate tuning of controller availability. Therefore a unified framework which allows common method of analysis for these seemingly unrelated different architectures is of key interest. However to the best of our knowledge such unified framework is not addressed in existing literature. 


%While the existing architectures \cite{mertoguno2019physics,xu2017bunshin,arroyo2019yolo} use different parameters and analysis approaches, verifying their applicability to arbitrary CPS and control synthesis for CPS adopting them require a unified framework and a more general analysis approach, which has not been addressed to the best of our knowledge.


In this paper, we propose a framework that unifies the simplex architecture, BFT++, and their variations. We then present a control policy synthesis with formal safety guarantee using our proposed framework, which applies to different architectures. In this paper we make the following specific contributions:
\begin{itemize}
    \item We construct a hybrid system to model CPS implementing the simplex, BFT++, and their variant architectures. We propose a framework that unifies these architectures.
    \item We derive the sufficient conditions for a control policy to satisfy safety with respect to a specified budget. 
    \item We propose an algorithm to compute a control policy that satisfies our derived conditions. Our proposed algorithm converges to a feasible solution, given its existence, within finite number of iterations.
    \item  We validate our proposed approach using a case study on lateral control of Boeing 747. We show that our proposed approach guarantees the safety of Boeing 747 with respect to the given budget constraint.
\end{itemize}

%In this context our previous work only considered reactive restart-based approach and for hard safety constraint. In this work we develop a unified model which captures the state-of-the-art resilient architectures and an analytical framework to design control policy that maintain safety for given budget constraint. 

The reminder of the paper is organized as follows. Section \ref{sec:related} presents related work. Section \ref{sec:preli} presents preliminary background. Section \ref{sec:system model} introduces the CPS model and presents the problem statement. Section \ref{sec:framework} gives our proposed framework. Section \ref{sec:analysis} presents our proposed solution approach. Section \ref{sec:simulation} contains a case a study and Section \ref{sec:conclusion} concludes the paper.

==> intro_v4.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Introduction}\label{sec:intro}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Cyber-physical systems (CPS) are subject to random failures and malicious cyber attacks, which have been reported in applications such as transportation \cite{Jeep} and power system \cite{case2016analysis}. The failures and attacks can potentially cause safety violation of the physical components, which will further lead to severe damage to the plants and harm to humans. 

To address random failures, the simplex architecture \cite{sha2001using} and its variants \cite{bak2009system,mohan2013s3a} are widely adopted. These architectures ensure safety by constraining the system states within an envelope using a safety controller, which is invoked when the main controller (also referred as high performance controller) incurs faults. This safety controller is assumed to be fault-free and is usually chosen from some well-established classical controllers. However an adversary may corrupt the safety controller through malicious attack and cause safety violations.

To provide safety and resilience against adversary, Byzantine fault tolerant++ (BFT++) architecture \cite{mertoguno2019physics} is proposed and already found application to different CPS \cite{xu2017bunshin,arroyo2019yolo}. BFT++ and its variations \cite{mertoguno2019physics,xu2017bunshin,arroyo2019yolo} utilize the fact that the physical subsystem follows the law of physics and has natural resilience against limited cyber disruptions due to difference of time scales in cyber and physical subsystems. 

Vanilla BFT++ \cite{mertoguno2019physics}, which is applied to CPS with redundant controllers, implements execution level diversity in the controllers to ensure that adversary can own only one controller while other ones crash upon attack. Using the crash as a signal, all the corrupted or crashed controllers are then restored from another redundant backup controller with appropriate delayed buffer so that its state remains uncorrupted. When the controllers are restored within the physical subsystem's natural resilience, the system's safety is guaranteed. BFT++ variations differ in their implementation of diversity and/or backup controllers \cite{xu2017bunshin}. For systems without redundant controllers, \cite{arroyo2019yolo} adopts proactive or periodic restart of the cyber components to recover the system from malicious attack. The physical subsystem can maintain safety by tuning controller availability.

However, due to disparity in implementation and timing behaviours among the above architectures, analyses undertaken for these architectures are seen to be quite distinct, and sometimes informal or restrictive in the sense that formal safety may not be guaranteed analytically for an arbitrary system. Therefore a unified framework which allows a common method of analysis for these seemingly unrelated different architectures is of key interest. This framework will also enable comparison among different architectures under a common baseline. However, how to construct a unified framework remains an open problem.


%to prevent the adversary from gaining foothold in the system. Similar idea is also applied in \cite{xu2017bunshin} at the program level. If the crashed controllers are restored fast enough, the physical subsystem can remain safe leveraging its resilience. Vanilla BFT++ \cite{mertoguno2019physics} achieves fast restoration by equipping the redundant backup controller with a delayed buffer whose size is properly tuned so that a good state to be recovered to is contained in it. When the system does not have redundant controllers, \cite{arroyo2019yolo} proactively restarts the cyber component so as to recover the system from malicious attack. The physical subsystem is shown to be safe if a minimum controller availability is guaranteed.



%The disparity in implementation and timing behaviours among these variants lead to distinct analysis for controller synthesis. 
%Therefore a unified framework which allows common method of analysis for these seemingly unrelated different architectures is of key interest. However to the best of our knowledge such unified framework is not addressed in the existing literature. 


%While the existing architectures \cite{mertoguno2019physics,xu2017bunshin,arroyo2019yolo} use different parameters and analysis approaches, verifying their applicability to arbitrary CPS and control synthesis for CPS adopting them require a unified framework and a more general analysis approach, which has not been addressed to the best of our knowledge.


In this paper, we propose a framework that unifies the simplex architecture, BFT++, and their variations. We then present a control policy synthesis with formal safety guarantee using our proposed framework, which applies to these different architectures. In this paper we make the following specific contributions:
\begin{itemize}
    \item We construct a hybrid system to model CPS implementing the simplex, BFT++, and their variant architectures. We propose a framework that unifies these architectures.
    \item We derive the sufficient conditions for a control policy to satisfy safety with respect to a specified budget. 
    \item We propose an algorithm to compute a control policy that satisfies our derived conditions. Our proposed algorithm converges to a feasible solution, given its existence, within finite number of iterations.
    \item  We validate our proposed approach using a case study on lateral control of Boeing 747. We show that our proposed approach guarantees the safety of Boeing 747 with respect to the given budget constraint.
\end{itemize}

%In this context our previous work only considered reactive restart-based approach and for hard safety constraint. In this work we develop a unified model which captures the state-of-the-art resilient architectures and an analytical framework to design control policy that maintain safety for given budget constraint. 

The reminder of the paper is organized as follows. Section \ref{sec:related} presents the related work. Section \ref{sec:system model} introduces the CPS model and presents the problem statement. Section \ref{sec:framework} gives our proposed framework. Section \ref{sec:analysis} presents our proposed solution approach. Section \ref{sec:simulation} contains a case a study and Section \ref{sec:conclusion} concludes the paper.

==> intro_v5.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Introduction}\label{sec:intro}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Cyber-physical systems (CPS) are subject to random failures and malicious cyber attacks, which have been reported in applications such as transportation \cite{Jeep} and power system \cite{case2016analysis}. Failures and attacks can potentially cause safety violation of the physical components, which will further lead to severe damage to the plants and harm to humans. 

%Random failures can occur independently in the unverified system components, which may lead to termination of the ability to function and further safety violation. To this end, fault tolerant control schemes \cite{zhang2008bibliographical,sharifi2010fault,xu2020distributed} and architectures such as the simplex architecture \cite{sha2001using,bak2009system,mohan2013s3a} have been proposed. These approaches have shown their success when some components in CPS are fault-free. This requirement, however, may not be practical for all CPS, especially those under malicious attacks.

Random failures can occur independently in the unverified system components, which causes termination of desired functions and may lead to safety violation. To this end, various fault tolerant control schemes \cite{zhang2008bibliographical,sharifi2010fault,xu2020distributed} and architectures such as the simplex architecture \cite{sha2001using,bak2009system,mohan2013s3a} have been proposed. These approaches are effective in CPS when some components are verified to be fault-free. This requirement, however, may not be viable for all CPS, especially those subject to malicious attacks.

A malicious adversary can exploit the vulnerabilities in the cyber subsystem and intrude into CPS. The adversary can then corrupt all the components in CPS making fault tolerant approaches ineffective. Various research efforts have been made to provide safety and resilience for CPS against adversary such as attack detection \cite{fawzi2014secure}, state reconstruction \cite{pajic2014robustness}, and resilience assessment \cite{clark2017cyber}. To strengthen the cyber security, an implementation fusing multiple versions of protection mechanisms was proposed in \cite{xu2017bunshin}. Until recently, a seminal work proposed a cyber resilient architecture, named Byzantine fault tolerant++ (BFT++) \cite{mertoguno2019physics}, for CPS under malicious cyber attacks. BFT++ as well as some other architectures (which we refer as BFT++ variants) \cite{mertoguno2019physics,xu2017bunshin,arroyo2019yolo} utilize the fact that the physical subsystem follows the law of physics and has natural resilience against limited cyber disruptions due to the difference of time scales in cyber and physical subsystems. 

BFT++ \cite{mertoguno2019physics}, which is applied to CPS with redundant controllers, uses one of the controller as backup. The other controllers are engineered to crash upon malicious attack, which further triggers automatic controller recovery using the backup. If the controllers are restored before saturating the physical subsystem's natural resilience, system safety is guaranteed. Another approach called YOLO \cite{arroyo2019yolo} is proposed when there is no redundant controller in CPS \cite{arroyo2019yolo}. The controller in YOLO is programmed to restart proactively or periodically to recover the system from malicious attack. The physical subsystem can then maintain safety by tuning controller availability.

However, due to disparity in implementation and timing behaviours among the BFT++ and its variants, analysis undertaken for these cyber resilient architectures are seen to be quite distinct, and sometimes informal or restrictive in the sense that formal safety may not be guaranteed analytically for an arbitrary system. Therefore a unified framework which allows a common method of analysis for these seemingly unrelated yet novel architectures is of key interest. This framework will also enable comparison among different architectures under a common baseline. Currently, however, such analytical framework does not exist.

In this paper, we propose a framework that unifies the simplex architecture, BFT++, and their variants. We then present a control policy synthesis with formal safety guarantee using our proposed framework, which applies to these different architectures. For convenience in this paper we interchangeably use BFT++ family or cyber resilient architectures to refer BFT++ and its variants. In this work we make the following specific contributions:
\begin{itemize}
    \item We construct a hybrid system to model CPS implementing the simplex and cyber resilient architectures. We propose a framework that unifies these architectures.
    \item We derive the sufficient conditions for a control policy to satisfy safety with respect to a specified budget. 
    \item We propose an algorithm to compute a control policy that satisfies our derived conditions. Our proposed algorithm converges to a feasible solution, given its existence, within finite number of iterations.
    \item  We validate our proposed approach using a case study on lateral control of Boeing 747. We show that our proposed approach guarantees the safety of Boeing 747 with respect to the given budget constraint.
\end{itemize}

%In this context our previous work only considered reactive restart-based approach and for hard safety constraint. In this work we develop a unified model which captures the state-of-the-art resilient architectures and an analytical framework to design control policy that maintain safety for given budget constraint. 

The reminder of the paper is organized as follows. Section \ref{sec:related} presents the related work. Section \ref{sec:system model} introduces the CPS model and presents the problem statement. Section \ref{sec:framework} gives our proposed framework. Section \ref{sec:analysis} presents our proposed solution approach. Section \ref{sec:simulation} contains a case a study on Boeing 747. Section \ref{sec:conclusion} concludes the paper.

==> prelim.tex <==
\section{Preliminary Background} \label{sec:preli}
This section gives preliminary background. 

Consider a continuous-time control-affine system
\begin{equation}\label{eq:dynamics}
    \dot{x}_t = f(x_t)+g(x_t)u_t,
\end{equation}
where $x_t\in \mathcal{X} \subset \mathbb{R}^n$ is the system state and $u_t\in\mathcal{U}\subset\mathbb{R}^m$ is the control input. Functions $f:\mathbb{R}^n\rightarrow\mathbb{R}^n$ and $g:\mathbb{R}^{n\times m}\rightarrow\mathbb{R}^n$ are assumed to be Lipschitz continuous. Let a set $\mathcal{C}$ be defined as $\mathcal{C}=\{x\in\mathcal{X}:h(x)\geq 0\}$, where function $h:\mathcal{X}\rightarrow\mathbb{R}$ is continuously differentiable. We say function $h$ is a zeroing control barrier function (ZCBF) if it satisfies the following definition.
\begin{definition}[Zeroing CBF (ZCBF) \cite{ames2016control}]\label{def:ZCBF}
Consider a dynamical system \eqref{eq:dynamics} and a continuously differentiable function $h:\mathcal{X}\rightarrow\mathbb{R}$. If there exists a locally Lipschitz extended class $\mathcal{K}$ function $\alpha$ such that  
\begin{equation}
    \sup_{u\in\mathcal{U}}\bigg\{\frac{\partial h(x)}{\partial x}f(x)+\frac{\partial h(x)}{\partial x}g(x)u
    +\alpha(h(x))\bigg\}\geq 0, \label{ZCBF_eqn}
\end{equation}
holds for all $x\in\mathcal{X}$, then function $h$ is a ZCBF.
\end{definition}
ZCBF provides a sufficient condition to guarantee the forward invariance of $\mathcal{C}$ as follows.
\begin{lemma}[\cite{ames2016control}]\label{lemma:ZCBF}
Given a dynamical system \eqref{eq:dynamics} and a set $\mathcal{C}=\{x\in\mathcal{X}:h(x)\geq0\}$, if $h$ is a ZCBF defined on $\mathcal{X}$, then $\mathcal{C}$ is forward invariant for any control $u$ satisfying \eqref{ZCBF_eqn}.
\end{lemma}

==> related.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Related Work}\label{sec:related}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Safety verification \cite{prajna2007framework,pajic2014safety} and safety controller synthesis \cite{ames2016control,cohen2020approximate,qin2021learning,herbert2017fastrack,chen2017reachability} for CPS operated in benign environment have been extensively studied. 

The simplex architecture \cite{sha2001using,bak2009system,mohan2013s3a} has been widely adopted for CPS that may incur faults. The simplex architecture consists of a main controller that is vulnerable to random failures and a safety controller that is verifiable and fault-free. Under certain conditions, e.g., the main controller incurs fault, a decision module instantaneously switches to the fault-free safety controller to control the system. Although the simplex architecture is easy to implement, it assumes that the faulty behaviors only happen within the main controller. When the system is under malicious attack, this assumption is violated since the adversary can corrupt all components.

Besides various control- and game-theoretic approaches aimed to prevent the system from malicious attacks \cite{pajic2014robustness,fawzi2014secure,cardenas2008research}, the family of BFT++ architectures \cite{mertoguno2019physics,arroyo2019yolo,xu2017bunshin} have attracted increasing research attention due to being practical to implement and agnostic to specific adversaries. The implementations of BFT++ and its variations are system dependent. For CPS with redundancy such as controllers \cite{mertoguno2019physics,xu2017bunshin}, the CPS can restore the controllers that crashed or are corrupted due to malicious attack using the redundant ones, which are equipped with a buffer that can be used to identify and flush out the malicious inputs. For CPS without redundancy, the controllers reboot either proactively \cite{arroyo2019yolo,abdi2018guaranteed} or reactively \cite{abdi2017application} to recover to a `clean' state. 

% Design of safe control policy along with an aforementioned architecture implemented to one system may not be easy and also may not hold to various systems since the tolerance by inertia and cyber setting are different. To this end, we propose a framework that unifies the aforementioned cyber resilient and simplex architectures, and develop a formal and general safety analysis on the proposed framework. We synthesize the control policy using a CBF-based approach, which was initially proposed in \cite{ames2014control}, to encode the safety controller synthesis problem as a sum-of-squares constraint. CBF-based approaches have also been applied to stochastic systems \cite{clark2021control}, sampled-data systems \cite{niu2021safety,singletary2020control}, and high relative degree \cite{xiao2019control}. 
 


==> related_v2.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Related Work}\label{sec:related}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Safety verification \cite{prajna2007framework,pajic2014safety} and safety controller synthesis \cite{ames2016control,cohen2020approximate,qin2021learning,herbert2017fastrack,chen2017reachability} for CPS operated in benign environment have been extensively studied. The simplex architecture and its variants are used to guarantee system safety when CPS incur random failures. However, these approaches may not be effective for CPS under malicious cyber attacks.

There exist two main trends of approaches to address CPS under malicious cyber attacks. The first category aims at preventing the system from malicious attacks using various control- and game-theoretic approaches \cite{pajic2014robustness,fawzi2014secure,cardenas2008research}. These approaches filter the impact introduced by the adversary. The second body of literature focuses on designing attack tolerant systems. BFT++ as well as its variants belong to this category. In parallel, restart- \cite{abdi2017application,abdi2018guaranteed} and software rejuventation-based mechanisms \cite{romagnoli2020software,arauz2021linear} are proposed for cyber intrusion tolerance. These mechanisms reset the cyber subsystem to a `clean' state via system level restart to recover from attack. The safety guarantee is achieved via system reachability analysis over bounded time, where the time bound depends on the restart frequency. 

In the present paper, we use an offline control barrier certificate-based analysis for control synthesis with formal safety guarantee \cite{prajna2007framework}. 
% The control barrier certificates and control policy are numerically solved using sum-of-squares (SOS) programs \cite{prajna2005sostools}.
Control barrier certificate-based approach has also been used in other applications such as safe coordination of multi-agent robotics \cite{borrmann2015control,wang2017safety}.

% Design of safe control policy along with an aforementioned architecture implemented to one system may not be easy and also may not hold to various systems since the tolerance by inertia and cyber setting are different. To this end, we propose a framework that unifies the aforementioned cyber resilient and simplex architectures, and develop a formal and general safety analysis on the proposed framework. We synthesize the control policy using a CBF-based approach, which was initially proposed in \cite{ames2014control}, to encode the safety controller synthesis problem as a sum-of-squares constraint. CBF-based approaches have also been applied to stochastic systems \cite{clark2021control}, sampled-data systems \cite{niu2021safety,singletary2020control}, and high relative degree \cite{xiao2019control}. 
 


==> sol.tex <==
\section{Control Barrier Function Based Control Synthesis}

Our solution approach consists of three steps. We first synthesize a finite time convergence CBF when the controller is in the normal state. We then synthesize a barrier certificate when the controller is in the corrupted and restoration/initialization state. We finally quantify the cost function incurred by the using the synthesized control policy.

\subsection{Control Synthesis in Normal State}

This subsection synthesizes the control policy when the controller is in the normal state. We will calculate the control policy using finite time convergence CBF based constraint. To this end, we first compute an FCBF following the approach proposed in \cite{clark2021verification}. 

\begin{lemma}\label{lemma:FCBF condition}
A function $b(x)$ is an FCBF if and only if there exists no $x$ satisfying $b(x)=0$, $\frac{\partial b}{\partial x}g(x)=0$, and $\frac{\partial b}{\partial x}f(x)<0.$
%% needs to be modified as following sufficient condition: $b(x)<=0$, $\frac{\partial b}{\partial x}g(x)=0$, and $\frac{\partial b}{\partial x}f(x)< \epsilon$ where $\epsilon$ is a positive number.
\end{lemma}
%%needs to modified according to modified Lemma 1
\begin{proof}
By the definition of FCBF, we have that $b(x)$ satisfies
\begin{equation*}
        \frac{\partial b(x)}{\partial x}(f(x)+g(x)u)+ \gamma\cdot sgn(b(x)) |b(x)|^\rho\geq 0.
\end{equation*}
When $\frac{\partial b}{\partial x}g(x)\neq 0$, we can choose $u$ as
\begin{equation*}
    u_i(t)=-\left(\left[\frac{\partial b}{\partial x}g(x)\right]_i\right)^{-1}\bigg(\gamma\cdot sgn(b(x)) |b(x)|^\rho
    +\frac{\partial b}{\partial x}f(x) \bigg).
\end{equation*}
When $\frac{\partial b}{\partial x}g(x)= 0$, if there exists $x$ such that $b(x)=0$ and 
\begin{equation*}
    \frac{\partial b}{\partial x}f(x)<0,
\end{equation*}
then $b(x)$ violates the definition.
\end{proof}

\begin{lemma}\label{lemma:FCBF synthesis}
A polynomial function $b(x)$ is an FCBF if and only if there exist polynomials $\beta(x)$ and $\theta_i(x)$, SOS polynomials $s_0(x)$ and $s_1(x)$, and integer $r$ such that
\begin{multline}\label{eq:positivstella encode}
    \beta(x)b(x) + \sum_{i=1}^m\theta_i(x)\left[\frac{\partial b}{\partial x}g(x)\right]_i\\
    -s_0(x)-s_1(x)\frac{\partial b}{\partial x}f(x)+ \left(\frac{\partial B}{\partial x}f(x)\right)^{2r}=0.
\end{multline}
where $i=1,\ldots,m$. Moreover, the set $\{x:b(x)\geq 0\}$ is a subset of the viability kernel of $\mathcal{C}=\{x:h(x)\geq 0\}$ if Eqn. \eqref{eq:positivstella encode} holds and there exists SOS polynomials $\iota_0(x)$, $\iota_1(x)$, and a polynomial $\omega(x)$ satisfying 
\begin{equation}\label{eq:viability condition}
    \iota_0(x)+\iota_1(x)b(x) +\omega(x)h(x)+1=0.
\end{equation}
\end{lemma}
\begin{proof}
The aim is to show that there exists a set of states $\{x:b(x)\geq 0\}$ such that
\begin{multline*}
    \{x:b(x)=0\}\cap\left(\cap_{i=1}^m\{x:\left[\frac{\partial b}{\partial x}g(x)\right]_i=0\}\right)\\
    \cap\left(\left\{x:\frac{\partial b}{\partial x}f(x)
    <0\right\}\right)=\emptyset
\end{multline*}
Using Positivstellensatz \cite{stengle1974nullstellensatz}, this is encoded as Eqn. \eqref{eq:positivstella encode}.

We next show $\{x:b(x)\geq 0\}$ is a subset of the viability kernel. Suppose there exists some $x_t\in\{x:b(x_t)\geq 0\}$ satisfying $x_t\notin\mathcal{C}$. Then there must exist some $x_{t'}$ for $t'<t$ such that $h(x_{t'})<0$ and $b(x_{t'})\geq 0$. Using Positivstellensatz, we have that if Eqn. \eqref{eq:viability condition} holds, then 
\begin{equation*}
    \{x:b(x)\geq 0\}\cap\{x:h(x)=0\}\cap\{x:1\neq 0\}=\emptyset,
\end{equation*}
indicating that such $x_{t'}$ does not exist.
\end{proof}

Given Lemma \ref{lemma:FCBF condition} and \ref{lemma:FCBF synthesis}, we can compute an FCBF using the general heuristic in \cite{clark2021verification}.

We denote the FCBF as $b(x)$. Then given parameters $\gamma>0$ and $\rho\in[0,1)$, we can compute a control input for each time $t$ as
\begin{subequations}\label{eq:control synthesis QP}
\begin{align}
    \min_{u}&\quad u^\top Qu\\
    \st&\quad  \frac{\partial b(x)}{\partial x}(f(x)+g(x)u)+ \gamma\cdot sgn(b(x)) |b(x)|^\rho\geq 0\label{eq:control synthesis QP constraint}
\end{align}
\end{subequations}
where $Q\in\mathbb{R}^{m\times m}$ is a positive definite matrix.

\subsection{Barrier Certificate Synthesis}
To obtain a control input during the normal mode, we need to guarantee that the quadratic program \eqref{eq:control synthesis QP} is always feasible. To this end, we synthesize a barrier certificate to guarantee the feasibility of Eqn. \eqref{eq:control synthesis QP}.

We define 
\begin{subequations}
\begin{align}
    l(x,u) &= \frac{\partial b}{\partial x}(f(x)+g(x)u)+ \gamma\cdot sgn(b(x)) |b(x)|^\rho,\\
    \mathcal{D}&=\{x:l(x,u)\geq 0 \text{ holds for some }u\},\\
    \mathcal{B}&=\{x:b(x)\geq 0\}.
\end{align}
\end{subequations}
We then synthesize a barrier certificate $v(x)$ to guarantee that $x_t\in\mathcal{D}$ during the corrupted and restoration states.
\begin{proposition}
Let $l(x,u)$ and $\mathcal{D}$ be as defined above. Consider BFT++ design. If there exist $\epsilon>0$ and a continuously differentiable function $v:\mathbb{R}^n\rightarrow\mathbb{R}$ such that
\begin{subequations}
\begin{align}
    &v(x)\geq \epsilon,~\forall x\in\mathcal{B}\label{eq:certificate 1}\\
    &v(x)\geq 0,~\forall x\in\mathcal{D}\label{eq:certificate 2}\\
    &v(x)<0,~\forall x\notin\mathcal{D}\label{eq:certificate 3}\\
    &\frac{\partial v}{\partial x}f(x)+\frac{\partial v}{\partial x}g(x)u\geq -\frac{\epsilon}{2\delta},~\forall (x,u)\in\mathbb{R}^n\times\mathbb{R}^m\label{eq:certificate 4}
\end{align}
\end{subequations}
where $\delta>0$ is the epoch length, then constraint \eqref{eq:control synthesis QP constraint} remains feasible for all $t$, regardless of the attack signal chosen by the adversary during the corrupted state and the delayed input during the restoration state.
\end{proposition}
\begin{proof}
We present a proof sketch in the following. Since the control signal during the normal state guarantees that the system reaches $\mathcal{B}$, Eqn. \eqref{eq:certificate 1} specifies the initial condition. By the BFT++ mechanism, the restoration lasts at most two epochs of time $2\delta$. By Eqn. \eqref{eq:certificate 4}, we have that during the restoration state, there does not exist some time $T$ such that $v(x_T)<0$. Then using Eqn. \eqref{eq:certificate 2}, we have that the system state belongs to $\mathcal{D}$ during the restoration state. By the definition of $\mathcal{D}$, we have that constraint \eqref{eq:control synthesis QP constraint} remains feasible.
\end{proof}
